How Well Can LLMs Negotiate? NegotiationArena Platform and Analysis

Negotiation is the basis of social interactions; humans negotiate everything from the price of cars to how to share common resources. With rapidly growing interest in using large language models (LLMs) to act as agents on behalf of human users, such LLM agents would also need to be able to negotiate. In this paper, we study how well LLMs can negotiate with each other. We develop NegotiationArena: a flexible framework for evaluating and probing the negotiation abilities of LLM agents. We implemented three types of scenarios in NegotiationArena to assess LLM's behaviors in allocating shared resources (ultimatum games), aggregate resources (trading games) and buy/sell goods (price negotiations). Each scenario allows for multiple turns of flexible dialogues between LLM agents to allow for more complex negotiations. Interestingly, LLM agents can significantly boost their negotiation outcomes by employing certain behavioral tactics. For example, by pretending to be desolate and desperate, LLMs can improve their payoffs by 20\% when negotiating against the standard GPT-4. We also quantify irrational negotiation behaviors exhibited by the LLM agents, many of which also appear in humans. Together, \NegotiationArena offers a new environment to investigate LLM interactions, enabling new insights into LLM's theory of mind, irrationality, and reasoning abilities.

==> scratchpad.tex <==
% We propose an arena for evaluating LLMA's behavior by situating them in games where they can negotiate, communicate, and exchange resources. 

% We measure the degree to which LLMs exhibit rational behavior, through various metrics such as game win rate, and investigation of player strategies when placed in different scenarios. 

% How might we measure the ability of LLMs to effectively communicate? Undoubtedly, it has become increasingly difficult to discern and measure progress toward this precisely. Measures of old, such as performance on NLP benchmarks \cite{wang-etal-2018-glue, hendryckstest2021, srivastava2023beyond}, are no longer sufficient --- partly due to intelligence and linguistic capacity often being confounded, and partly due to data/benchmark leaking \cite{aiyappa-etal-2023-trust, sainz-etal-2023-nlp,Li2023AnOS} (i.e., training on the test set). Better measures of progress are needed.


% Touted as a productive gauge of intelligence and coveted as a property of an intelligent agent \cite{RUSSELL199757}, we argue that studying rational behavior in agents is one possible approach. Rational agents reason and communicate effectively to reach their goals. AI agents should likewise do the same. A rational AI agent should be able to effectively comprehend its task and leverage its existing knowledge to attain its goal. While some recent work in the field explores how agents communicate, debate, and negotiate with each other~\cite{}, a flexible reference benchmark to compare different agents on negotiation is still missing.



% Our main finding is that while agents appear to follow rational behaviors, prompting them with social behaviors or personas can change the final payoffs; moreover, we find anchoring bias and lack of generalization capabilities in different games.


% For example, how often does an LLM agent propose trades that allow it to achieve its objective? 

% We believe that these games will be useful in studying not just how agents negotiate but generally exploring a wide range of behaviors:

% \begin{itemize}
%     \item \textbf{Rationality.} Negotiations provide a flexible and controllable environment to analyze agent rationality from economic and game theoretic perspectives, over a range of diverse scenarios. 
%     % Agents will interact in an environment where they can only partially observe the state (i.e., they don't know the other player's state). This will force them to define strategies that take unknown states into account. \mert{ is this a property of a rational agent? I think an irrational agent can also take unobserved states into account and still can make irrational decisions.}
%     \item \textbf{Social Behavior.} How agent behaves has an impact on how they tackle tasks. Hostile agents will be more aggressive in communication, affecting the result of the trades.
%     \item \textbf{Theory of Mind.} At each step, we can inspect agent behavior and ask the agent what they plan to do and what they think the other player has. Defining correct strategies also comes from imagining other players' motives.
%     \item \textbf{Counterfactual Reasoning} Since all the agents' conversations are saved as a structured object, we can any point in any conversation, change one or multiple words of one reply, and then replay the conversation from that exact point.
% \end{itemize}

% \mert{Is this the end of the intro? I think would be good to have a concluding paragraph / a few sentences. e.g. how our benchmark is a good start as a dynamical benchmark for evaluating rational behavior, organic evaluation of LLM abilities / comparisons etc etc}



% \subsection{Game Settings}

% \paragraph{Resource Exchange Game}
% The first agent is assigned 25 Xs and 5 Ys; the second agent is assigned 5 Xs and 25 Ys. Both agents are tasked with the goal of \textit{maximizing their overall resources}. They have \fede{add} number of turns to do so. 

% \paragraph{Ultimatum Game}

% The first agent is assigned 100 dollars and is the first to propose an initial possible split. The second agent, the Decider, will accept or propose a new trade. They have \fede{add} number of turns to find an agreement. Note that this makes this game different from the classical ultimatum game, where only one turn exists.

% \paragraph{Seller and Buyer Game} 
% The first agent is assigned an object X to sell, and the second one has 100 ZUP (our imaginary currency) to buy it.  Agents have two different monetary valuations for the object and we test two different scenarios. In the first scenario, the seller's cost to make the object is 60 ZUP, while the buyer wants to pay at most 40 ZUP (hard agreement setting). The second scenario is the opposite: the seller's cost was 40 ZUP and the buyer wants to spend, at most, 60 ZUP (easy agreement setting). They have \fede{add} turns to do so.


